Texture-enhanced Light Field Super-resolution with Spatio-Angular Decomposition Kernels

Despite the recent progress in light field super-resolution (LFSR) achieved by convolutional neural networks, the correlation information of light field (LF) images has not been sufficiently studied and exploited due to the complexity of 4D LF data. To cope with such high-dimensional LF data, most of the existing LFSR methods resorted to decomposing it into lower dimensions and subsequently performing optimization on the decomposed sub-spaces. However, these methods are inherently limited as they neglected the characteristics of the decomposition operations and only utilized a limited set of LF sub-spaces ending up failing to sufficiently extract spatio-angular features and leading to a performance bottleneck. To overcome these limitations, in this paper, we comprehensively discover the potentials of LF decomposition and propose a novel concept of decomposition kernels. In particular, we systematically unify the decomposition operations of various sub-spaces into a series of such decomposition kernels, which are incorporated into our proposed Decomposition Kernel Network (DKNet) for comprehensive spatio-angular feature extraction. The proposed DKNet is experimentally verified to achieve considerable improvements compared with the state-of-the-art methods. To further improve DKNet in producing more visually pleasing LFSR results, based on the VGG network, we propose a LFVGG loss to guide the Texture-Enhanced DKNet (TE-DKNet) to generate rich authentic textures and enhance LF images' visual quality significantly. We also propose an indirect evaluation metric by taking advantage of LF material recognition to objectively assess the perceptual enhancement brought by the LFVGG loss.

==> tex/sections/bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,keepaspectratio]{images/authors/ZexiHu.jpg}}]{Zexi Hu} 
received his Bachelor's degree from South China Agricultural University, China in 2014 and his M.Phil. degree from the University of Sydney in 2017. He is now a Ph.D. student at the School of Computer Science, University of Sydney, Australia. His research focuses on image processing and deep learning.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,keepaspectratio]{images/authors/XiaomingChen.jpg}}] {Xiaoming Chen} received the B.Sc. degree from the Royal Melbourne Institute of Technology, Australia, in 2004, and the Ph.D. degree from the University of Sydney, Australia, in 2009. His research interests include immersive media computing, virtual reality, and related business information systems and applications. His work has been published in journals and conferences including IEEE Trans. on Image Processing, IEEE Trans. on Circuits and Systems for Video Technology, IEEE Trans. on Instrumentation and Measurement, ECCV, etc.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,keepaspectratio]{images/authors/HenryWingFungYeung.png}}] {Henry Wing Fung Yeung} received the M.Phil. degree in Engineering and IT from the University of Sydney, where he is currently pursuing the Ph.D. degree in Engineering and IT. His research interests include light field image processing and deep learning.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,keepaspectratio]{images/authors/YukYingChung.jpg}}] {Yuk Ying Chung} (M’05) received her B.S. degree in Computing and Information Systems from the University of London, UK, in 1995; and her Ph.D. degree in Computer Engineering from the Queensland University of Technology, Australia in 2000. She is a Senior Lecturer and has been with the School of Computer Science, University of Sydney, Australia since 2001. Her research interests include image and video processing, virtual reality and data mining. Her work has been published in conferences and journals including ECCV, NeurIPS, IEEE Trans. on Image Processing, and IEEE Trans. on Circuits and Systems for Video Technology, IEEE Trans. on Cybernetics, etc.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,keepaspectratio]{images/authors/ZhiboChen.jpeg}}] {Zhibo Chen} (M’01–SM’11) received the B.S. and Ph.D. degrees from Department of Electrical Engineering, Tsinghua University, Beijing, China, in 1998 and 2003, respectively. He is now a professor in the University of Science and Technology of China. His research interests include image and video compression, visual quality of experience assessment, immersive media computing, and intelligent media computing. He has more than 100 publications and more than 50 granted EU and US patents. He is the Secretary of IEEE Visual Signal Processing and Communications Committee, and a member of IEEE Multimedia System and Applications Committee. He was a TPC chair of PCS 2019 and a organization committee member of ICIP 2017 and ICME 2013, and a TPC member of IEEE ISCAS and IEEE VCIP.
\end{IEEEbiography}

==> tex/table/PerfDenseConn.tex <==
\begin{table*}[ht]
    \caption{Study of dense and raw image connections on $4 \times$ scale. The best item of each decomposition kernel is underlined.}
    \label{tab:PerfDenseConn}
    \centering
    % \resizebox{\textwidth}{!}{
    \begin{tabu}{|l||c|c|c|c||c|c|c|c|}
        \hline
        \rule{0pt}{8pt}Kernel       & \multicolumn{4}{c||}{$\mathcal{K}^{\gamma}$} & \multicolumn{4}{c|}{$\mathcal{K}^{SAS}$} \\ \hline
        Dense Connections           & \xmark                 & \xmark                  & \cmark                    & \cmark                      & \xmark      & \xmark   & \cmark   & \cmark               \\ \hline
        Raw Image Connections       & \xmark                 & \cmark                  & \xmark                    & \cmark                      & \xmark      & \cmark   & \xmark   & \cmark               \\ \hline
        PSNR                        & 15.54                  & 34.80                   & 35.52                     & \underline{36.07}           & 15.52       & 34.50    & 35.01    & \underline{35.55}    \\ \hline
        SSIM                        & 0.2712                 & 0.9671                  & 0.9724                    & \underline{0.9752}          & 0.2710      & 0.9647   & 0.9680   & \underline{0.9724}   \\ \hline
    \end{tabu}
    % }
\end{table*}

==> tex/table/PerfL.tex <==
\begin{table*}[ht]
    \caption{Study of numbers of decomposition kernels $L$ on $4 \times$ scale. The best item is underlined.}
    \label{tab:PerfL}
    \tabcolsep=0.08cm
    \centering
    % \resizebox{\textwidth}{!}{
        \begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
        \hline
        $L$     & 2         & 3         & 4         & 5         & 6         & 7         & 8         & 9         & 10        & 11        & 12        & 13        & 14        & 15        & 16        & 17        & 18                    & 19        \\ \hline
        PSNR    & 34.59     & 34.95     & 35.10     & 35.12     & 35.46     & 35.52     & 35.53     & 35.64     & 35.66     & 35.68     & 35.72     & 35.74     & 35.85     & 35.90     & 35.91     & 36.00     & \underline{36.07}     & 35.84     \\ \hline
        SSIM    & 0.9652    & 0.9688    & 0.9695    & 0.9695    & 0.9718    & 0.9722    & 0.9721    & 0.9729    & 0.9731    & 0.9731    & 0.9733    & 0.9735    & 0.9742    & 0.9744    & 0.9744    & 0.9748    & \underline{0.9752}    & 0.9734    \\ \hline
        \end{tabular}
    % }
\end{table*}
